Including van der Waals Forces in Diffusion-Convection Equations - Modeling, Analysis, and Numerical Simulations

This paper presents a model of van der Waals forces in the framework of diffusion-convection equations. The model consists of a nonlinear and degenerated diffusion-convection equation, which furthermore can be considered as a model for slow perikinetic coagulation. For the analytical investigation, we transform the model to a porous medium equation, which provides us access to the comprehensive analytical results for porous medium equations. Additionally, this transformation reveals a new application for porous medium equations. Eventually, we present numerical simulations of the model by solving the porous medium equation. We note that we solve the porous medium equation without any further regularization, which is often applied in this context.

==> environments_paper.tex <==
\usepackage{amsthm}         % math theorem environments

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 1.1 Define theorem environments -- environments with italic letters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}    
   %Theorem
   \crefformat{thm}{Theorem~#2#1#3}                %define citation format for counter "thm"
   \newtheorem{thm}{Theorem}[section]              %define new environment "thm" that automatically creates a counter "thm". Choose numbering subordinate to chapters    
   \crefname{thm}{Theorem}{Theorems}               %define single/plural citation names for environment "thm"
   %Proposition    
   \crefformat{count_prop}{Proposition~#2#1#3}        %define citation format for counter "count_prop"
   \newaliascnt{count_prop}{thm}                      %define counter "count_prop" as a alias for the counter "thm". This enables consecutive numbering.
   \newtheorem{proposition}[count_prop]{Proposition}  %define new environment "proposition" that uses the counter "count_prop" with the above specified citation format 
   \aliascntresetthe{count_prop}                      %close definition
   \crefname{proposition}{Proposition}{Propositions}  %define single/plural citation names for environment "proposition"
   %Lemma 
   \crefformat{count_lem}{Lemma~#2#1#3}       
   \newaliascnt{count_lem}{thm}               
   \newtheorem{lemma}[count_lem]{Lemma}        
   \aliascntresetthe{count_lem}                
   \crefname{lemma}{Lemma}{Lemmas}
   %Definition
   \crefformat{count_defi}{Definition~#2#1#3}       
   \newaliascnt{count_defi}{thm}
   \newtheorem{definition}[count_defi]{Definition}
   \aliascntresetthe{count_defi}                
   \crefname{definition}{Definition}{Definitions}
   %Corollary
   \crefformat{count_cor}{Corollary~#2#1#3}       
   \newaliascnt{count_cor}{thm}
   \newtheorem{corollary}[count_cor]{Corollary} 
   \aliascntresetthe{count_cor}                
   \crefname{corollary}{Corollary}{Corollaries}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 1.2 Define theorem environments -- environments with normal letters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{definition}  
   %Remark                        
   \crefformat{count_rem}{Remark~#2#1#3}       
   \newaliascnt{count_rem}{thm}
   \newtheorem{remark}[count_rem]{Remark}
   \aliascntresetthe{count_rem}                
   \crefname{remark}{Remark}{Remarks}
    %Example
   \crefformat{count_exmpl}{Example~#2#1#3}       
   \newaliascnt{count_exmpl}{thm}
   \newtheorem{example}[count_exmpl]{Example}
   \aliascntresetthe{count_exmpl}                
   \crefname{example}{Example}{Examples}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 2. Define reference layout for different environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\crefname{figure}{Figure}{Figures}
\crefname{algorithm}{Algorithm}{Algorithms}
\crefname{subsection}{Section}{Section}
\crefname{section}{Section}{Section}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 3. Define new environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Proof environment
\newenvironment{Proof}[1][{\noindent\textbf{Proof:~~}}]{ {#1}}{\hfill$\square$}

==> mathmacros_paper.tex <==
%===========================================================================================
%===========================================================================================
%
%  I   GLOBAL MATHEMATICAL MACROS 
%
%===========================================================================================
%===========================================================================================
\usepackage{xargs}   %usepackage for macros with several default parameters


%==================================================
%  I.1  Names and Words
%==================================================
%names
\newcommand{\vdW}{van der Waals}
\newcommand{\Avogadro}{Avogadro}
\newcommand{\Grown}{Grownwall's inequality}
\newcommand{\Holder}{H\"{o}lder's inequality}
\newcommand{\Lifshitz}{Lifshitz}


%word macros for constistent writing 
%\newcommand{\theorem}{\ensuremath{ \textnormal{Theorem} }}
\newcommand{\Lemma}{Lemma}
\newcommand{\Definition}{Definition}


%==================================================
%   I.2  Mathematical terms
%==================================================
\newcommand{\Div}{\ensuremath{ \textnormal{div} }}                               
\newcommand{\mol}{\ensuremath{ \textit{mol} }} 
                                               
%%==================================================
%  I.3  Greek Letters
%==================================================
%capture misspelling
\newcommand{\lamdba}{\ensuremath{ \lambda }}
%shortcuts             
\newcommand{\vphi}{\ensuremath{ \varphi }}                      
\newcommand{\veps}{\ensuremath{ \varepsilon }}
\newcommand{\eps}{\ensuremath{ \epsilon }}


%==================================================
%  I.4  Set of Numbers
%==================================================
\newcommand{\setN}{\ensuremath{ \mathbb{N} }}                   
\newcommand{\setZ}{\ensuremath{ \mathbb{Z} }}                   
\newcommand{\setR}{\ensuremath{ \mathbb{R} }}                   
\newcommand{\setC}{\ensuremath{ \mathbb{C} }}                                                           


%==================================================
%  I.5  Brackets and arrows
%==================================================
%bracket: \brac{xx}
\newcommand*{\brac}[1]{\ensuremath{ \left( {#1} \right) }}                          
%squared bracket: \sqbrac{xx}
\newcommand*{\sqbrac}[1]{\ensuremath{ \left[ {#1} \right] }}                         
%curly bracket \cbrac{xx}
\newcommand*{\cbrac}[1]{\ensuremath{ \left\{ {#1} \right\} }}                        

%Implication arrows with more spacing 
\newcommand*{\hence}{\ensuremath{ ~~\Rightarrow~~ }} 
\newcommand*{\Hence}{\ensuremath{ ~~\Longrightarrow~~ }} 
%Equivalence arrows with more spacing 
\newcommand*{\equivalent}{\ensuremath{ ~~\Leftrightarrow~~ }}                                                                                                                            
\newcommand*{\Equivalent}{\ensuremath{ ~~\Longleftrightarrow~~ }}  


%==================================================
%  I.6  Vectors and Norms for Vectors
%==================================================
%Vector: \vec{xx}             Example: \vec{v}
\renewcommand*{\vec}[1]{ \ensuremath{ \boldsymbol{#1} }}

%Vectornorm: \abs[opt]{xx}    Examples \abs{\vec{v}}  \abs[2]{\vec{v}}
\newcommand*{\abs}[1]{\left| {#1} \right| }

%Vectornorm: Eucledian norm
\newcommand*{\absE}[1]{\left| {#1} \right|_2 }
%Vectornorm: Forbenius norm
\newcommand*{\absF}[1]{\left| {#1} \right|_F }


%==================================================
%  I.7  Products on Banach spaces        
%==================================================
%sets two objects in scalarproduct:  \scp{x}{x}       
\newcommand*{\scp}[2]{\ensuremath{ \left( {#1}~,~{#2} \right) }}    
%sets two objects in dual pairing:   \dualp{x}{x}   
\newcommand*{\dualp}[2]{\ensuremath{ \left\langle {#1}~,~{#2} \right\rangle }}       


%==================================================
%  I.8  Dervivatives
%==================================================
%Gradient: \grad 
\newcommand*{\grad}{\vec{\nabla}\!}
%Directional derivative: \derd[opt]
\newcommand*{\derd}[1][i]{\ensuremath{ \partial_{{#1}} }}
%Temporal derivative: \dert[opt]            
\newcommand*{\dert}[1][t]{\ensuremath{ \partial_{{#1}} }}
%Material derivative: \derm[opt]
\newcommand*{\derm}[1][t]{\ensuremath{ \frac{D}{D{#1}} }} 
%dervative on real line: \derr[opt]
\newcommand*{\derr}[1][x]{\ensuremath{ \frac{d}{d{#1}} }}


%==================================================
%  I.9  Integrals
%==================================================
%Define mean value integral:  \mwint 
\DeclareMathOperator*{\mwint}{\textbf{--}\!\!\!\!\!\!\int} 

%Integral:   \Int{integrand variable}{subscript}{superscript}{function}  
\newcommand{\Int}[4]{\ensuremath{ \int\limits_{#2}^{{#3}} {#4} d{#1} }}    
%Volume integral with respect to dx and defaluft domain:  \Intdx[domain]{function}
\newcommand*{\Intdx}[2][\Omega]{ \Int{x}{{#1}}{}{{#2}} } 
%Surface integral with respect to dS and default domain: \IntdS[domain]{function}
\newcommand*{\IntdS}[2][\Gamma]{ \Int{S}{{#1}}{}{{#2}} }            
%Time integral with respect to dt and default interval:    \Intdt[lower border][upper border]{function}
\newcommandx*{\Intdt}[3][1=0,2=T,usedefault]{ \Int{t}{{#1}}{{#2}}{{#3}} }  


%======================================================
%  I.10  Function Spaces and Norms of Function Spaces
%======================================================
%Function sapce: \fspace[hspace]{name}{domain}{range}        Examples: \fspace{L^p}{\Omega}{}    \fspace[-3pt]{C^0}{[0,T]}{;V}
\newcommandx*{\fspace}[4][1=-1pt,usedefault]{ \ensuremath{  {{#2}} \hspace{#1} \left( {#3}{#4} \right) }}
%Norms for functions: \norm{object}{space}                    Examples: \norm{f}{L^2} \norm{\vec{u}}{\setR^n}
\newcommandx*{\norm}[2]{ \ensuremath{ \left\| {#1} \right\|_{{#2}}   }}

%========================================
%  I.10.1   Ck Spaces        
%========================================
%\Ck[domain][subscript]{smoothness k}{range}                  Examples: \Ck{0,\alpha}{}    \Ck[D]{0}{;V}  \Ck[][\loc]{0}{;V}^*
\newcommandx*{\Ck}[4][1=\Omega,2= ,usedefault]{ \fspace{ C^{{#3}}_{{#2}} }{ {#1} }{ {#4} } }

%========================================
%  I.10.2   Lp Spaces        
%========================================
%\Ck[domain][subscript]{exponent p}{range}                    Examples: \Lp{p}{} \Lp[D]{p}{;\setR^N}    \Lp[][\loc]{p}{;V}^*
\newcommandx*{\Lp}[4][1=\Omega,2= ,usedefault]{ \fspace{ L^{{#3}}_{{#2}} }{ {#1} }{ {#4} } }

%========================================
%  I.10.3  Sobolev Spaces        
%========================================
%\Wkp[domain][subscript]{smoothness k}{exponent p}{range}     Examples: \Wkp{1}{2}{}  \Wkp[D]{1}{p}{;\setR^N}    \Wkp[][\loc]{1}{p}{}  \Wkp[][\loc]{1}{p}{;V}^*
\newcommandx*{\Wkp}[5][1=\Omega,2= ,usedefault]{ \fspace{ W^{{#3},{#4}}_{{#2}} }{ {#1} }{ {#5} } }
%\Hk[domain][subscript]{smoothness k}{range}                  Examples: \Hk{1}{}  \Hk[D]{1}{;\setR^N}    \Hk[][\loc]{1}{}  \Hk[][\loc]{1}{;V}^*
\newcommandx*{\Hk}[4][1=\Omega,2= ,usedefault]{ \fspace{ H^{{#3}}_{{#2}} }{ {#1} }{ {#4} } }
  %\Hkdiv[domain][subscript]{smoothness k}                    Examples: \Hkdiv{}  \Hkdiv[D]{k}    \Hkdiv[][f]{k}  \Hkdiv[D][\loc]{1}^*
\newcommandx*{\Hkdiv}[3][1=\Omega,2= ,usedefault]{ \fspace{ H^{{#3}}_{{#2}} }{\Div}{;{#1}} }



%===========================================================================================
%===========================================================================================
%
%  II   MATHEMATICAL MACROS FOR CURRENT PAPER
%
%===========================================================================================
%===========================================================================================


%==============================================
%  11.1  Shortcuts for frequently used names
%==============================================
\newcommand{\concentration}{number concentration}
\newcommand{\concentrationMol}{molar concentration}
\newcommand{\massflux}{number mass flux}
\newcommand{\massfluxMol}{molar mass flux}
\newcommand*{\dnpp}{\textnormal{DNPP-system}}
\newcommand*{\snpp}{\textnormal{SNPP-system}}


%==================================================
%  11.2  Shortcuts for frequently used vectors
%================================================== 
\newcommand*{\vecc}{\vec{c}}
\newcommand*{\vecg}{\vec{g}}
\newcommand*{\vecu}{\vec{u}}
\newcommand*{\vecv}{\vec{v}}
\newcommand*{\vecj}{\vec{j}}
\newcommand*{\vecJ}{\vec{J}}
\newcommand*{\vecnu}{\vec{\nu}}
\newcommand*{\vecF}{\vec{F}}
\newcommand*{\vecE}{\vec{E}}


%==================================================
%  II.3  Frequently used sets
%==================================================
%Parabolic cylinder: \OmegaT 
\newcommand*{\OmegaT}[1][T]{\ensuremath{ \Omega_{#1} }}
%Parabolic boundary: \GammaT
\newcommand*{\GammaT}[1][T]{\ensuremath{ \Gamma_{#1} }}  


%==================================================
%  11.4  Variables of the considered System
%==================================================
%General continuous variables
\newcommand*{\tx}{(t,x)}

% Physical units: number concentration
\newcommand{\unitConc}{ \sqbrac{m^{-3}} }
% Physical units: number concentration
\newcommand{\unitConcMol}{ \sqbrac{mol\,m^{-3}} }
% Physical units: number mass flux
\newcommand{\unitFlux}{ \sqbrac{m^{-2}s^{-1}} }
% Physical units: molar mass flux
\newcommand{\unitFluxMol}{ \sqbrac{mol\,m^{-2}s^{-1}} }
% Physical units: PDE for number concentration
\newcommand{\unitPDE}{ \sqbrac{m^{-3}s^{-1}} }
% Physical units: PDE for molar concentration
\newcommand{\unitPDEMol}{ \sqbrac{mol\,m^{-3}s^{-1}} }

% Parameters: Diffusion coefficient
\newcommand*{\dl}[1][]{\ensuremath{ d_{{#1}} }}
% Parameters: mobility
\newcommand*{\mob}[1][]{\ensuremath{ \omega_{{#1}} }}
% Parameters: Electric permittivity
\newcommand*{\permitEL}{\ensuremath{ \epsilon }}


%Velocity: Flow field
\newcommand{\fieldFlow}{\ensuremath{ \vecu }}

% Number concentrations: l-th concentration
\newcommand{\nl}[1][]{\ensuremath{ c_{*{#1}} }}
% Number concentrations: gradient of l-th concentration
\newcommand{\nlgrad}[1][]{\ensuremath{ \grad\nl[{#1}] }}
% Number concentrations: Initial value for l-th concentration
\newcommand{\nlstart}[1][]{\ensuremath{ c_{*,0{#1}} }}
% Number concentrations: number mass flux of l-th concentration
\newcommand{\nlflux}[1][]{\ensuremath{ \vecJ_{*{#1}} }}
% Number concentrations: relative number mass flux of l-th concentration
\newcommand{\nlfluxrel}[1][]{\ensuremath{ \vecj_{*{#1}} }}
% Number concentrations: charge of l-th concentration  
\newcommand{\nlcharge}[1][l]{\ensuremath{ \zl[{#1}]\nl[{#1}] }}

% Molar concentrations: l-th concentration
\newcommand{\cl}[1][]{\ensuremath{ c_{{#1}} }}
% Molar concentrations: gradient of l-th concentration
\newcommand{\clgrad}[1][]{\ensuremath{ \grad\cl[{#1}] }}
% Molar concentrations: Initial value for l-th concentration
\newcommand{\clstart}[1][]{\ensuremath{ c_{0{#1}} }}
% Molar concentrations: molar mass flux of l-th concentration
\newcommand{\clflux}[1][]{\ensuremath{ \vecj_{{#1}} }}
% Molar concentrations: charge of l-th concentration  
\newcommand{\clcharge}[1][l]{\ensuremath{ \zl[{#1}]\cl[{#1}] }}

%Reaction rate functions
\newcommand{\Rl}[1][]{\ensuremath{ R_{{#1}} }}
                         
%Test function: Gradient of test function
\newcommand*{\gradphi}{\ensuremath{ \grad\vphi }}


%=====================================================================
%  II.5  Shortcuts for frequently used spaces
%=====================================================================  
%Concentrations: Test function space
\newcommand{\spaceT}{ \Hk[][0]{1}{} }
\newcommand{\spaceTh}{ V_h }
%Concentrations: Solution space
\newcommand{\spaceS}{ \fspace{L^2}{I}{; \spaceT } \cap \fspace{H^1}{I}{; \spaceT^* } }
%Concentrations: Abbreviation for solution space
\newcommand{\spaceSshort}{ X }
